Updated analysis of NN elastic scattering to 3 GeV

A partial-wave analysis of NN elastic scattering data has been updated to include a number of recent measurements. Experiments carried out at the Cooler Synchrotron (COSY) by the EDDA Collaboration have had a significant impact above 1 GeV. Results are discussed in terms of the partial-wave and direct-reconstruction amplitudes.

==> Makefile.latex <==
BIB_FILES=../../gwu.bib
PAPER=letter

all:    nn07_4.pdf

%.aux : %.tex
	latex $<

%.bbl : %.aux $(BIB_FILES)
	bibtex $<

%.pdf: %.tex 
	latex $<; latex $<
	dvipdfm -p $(PAPER) $*.dvi
	rm -f *.{log,dvi,ps,toc,blg,aux}

clean:
	rm -f *.{pdf,log,dvi,ps,aux,toc,blg,bbl}

